Progress in Mathematical Programming Solvers from 2001 to 2020

This study investigates the progress made in LP and MILP solver performance during the last two decades by comparing the solver software from the beginning of the millennium with the codes available today. On average, we found out that for solving LP/MILP, computer hardware got about 20 times faster, and the algorithms improved by a factor of about nine for LP and around 50 for MILP, which gives a total speed-up of about 180 and 1,000 times, respectively. However, these numbers have a very high variance and they considerably underestimate the progress made on the algorithmic side: many problem instances can nowadays be solved within seconds, which the old codes are not able to solve within any reasonable time.

==> LP_table_tex_sorted.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
Name & nrows & ncols & nonzeros &  \oldS &  \newS & ratio  \\
\hline
chromaticindex1024-7 &      67583 &      73728 &     270324 &     4.0 &    1.4 &  2.9 \\
cont11\_lp            &     160792 &     120793 &     440387 &   984.8 &   13.8 & 71.4 \\
cont1\_lp             &     160792 &      80795 &     440387 &   151.8 &    7.0 & 21.7 \\
cont4\_lp             &     160792 &      80795 &     438795 &    27.6 &    7.0 &  3.9 \\
Daniel\_LP1           &     770997 &     814786 &    2908590 &    37.0 &   10.0 &  3.7 \\
Daniel\_LP2           &    3189051 &    3372988 &   11432557 &   344.7 &   73.4 &  4.7 \\
Daniel\_LP3           &    3189051 &    3372988 &   11432557 &   344.4 &   73.5 &  4.7 \\
dano3mip\_lp          &       3202 &      13873 &      79655 &     3.0 &    0.3 & 10.0 \\
datt256\_lp           &      11077 &     262144 &    1503732 &   319.6 &  170.8 &  1.9 \\
dbic1\_lp             &      43200 &     183235 &    1038761 &    12.8 &    3.0 &  4.3 \\
dfl001               &       6071 &      12230 &      35632 &     2.2 &    0.3 &  7.3 \\
%ds-big               &       1042 &     174997 &    4623442 &    21.6 &    8.0 &  2.7 \\
ds-big\_lp            &       1042 &     174997 &    4623442 &    11.8 &    3.9 &  3.0 \\
ex10                 &      69608 &      17680 &    1162000 &    78.0 &    2.4 & 32.5 \\
fhnw-binschedule0\_lp &      58085 &     319319 &    1382972 &    28.0 &    1.9 & 14.7 \\
fome12\_lp            &      24284 &      48920 &     142528 &    10.0 &    0.7 & 14.3 \\
fome13\_lp            &      48568 &      97840 &     285056 &    20.0 &    1.0 & 20.0 \\
graph40-40\_lp        &     360900 &     102600 &    1260900 &    93.7 &   15.6 &  6.0 \\
irish-electricity    &     104259 &      61728 &     523257 &    24.0 &    3.0 &  8.0 \\
ken-18\_lp            &     105127 &     154699 &     358171 &     1.8 &    0.9 &  2.0 \\
% ken-18.mps\_lp        &     105127 &     154699 &     358171 &     1.8 &    0.9 &  2.0 \\
L1\_sixm250obs\_lp     &     986069 &     428032 &    4280320 &   233.2 &    2.0 & 116.6 \\
l30\_lp               &       2701 &      15380 &      51169 &     1.0 &    0.3 &  3.3 \\
Linf\_520c\_lp         &      93326 &      69004 &     566193 &  2242.2 &    7.3 & 307.1 \\
lp22\_lp              &       2958 &      13434 &      65560 &     1.8 &    0.3 &  6.0 \\
mod2\_lp              &      34774 &      31728 &     165129 &     3.0 &    0.9 &  3.3 \\
neos1\_lp             &     131581 &       1892 &     468009 &     9.0 &    0.3 & 30.0 \\
neos2\_lp             &     132568 &       1560 &     552519 &     5.5 &    0.7 &  7.9 \\
neos-3025225\_lp      &      91572 &      69846 &    9357951 &    72.0 &   15.0 &  4.8 \\
neos3\_lp             &     512209 &       6624 &    1542816 &    87.1 &    0.8 & 108.9 \\
neos-5052403-cygnet  &      38268 &      32868 &    4898304 &    29.8 &    4.5 &  6.6 \\
neos-5251015\_lp      &     486531 &     136971 &    1955388 &    32.0 &    2.0 & 16.0 \\
\hline
\end{tabular}
\label{tab:LP-instances}
\caption{Problem size, run times of virtual Best  \oldS and \newS, and the ratio  \oldS/\newS of LP instances - Part I}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
Name & nrows & ncols & nonzeros &  \oldS &  \newS & ratio  \\
\hline
neos\_lp              &     479119 &      36786 &    1047675 &    43.5 &    5.1 &  8.5 \\
ns1644855\_lp         &      40698 &      40200 &    2120696 &    33.3 &    6.5 &  5.1 \\
ns1688926\_lp         &      32768 &      16587 &    1712128 &     7.0 &    1.0 &  7.0 \\
nug08-3rd\_lp         &      19728 &      20448 &     139008 &   278.4 &    4.0 & 69.6 \\
nug15\_lp             &       6330 &      22275 &      94950 &    34.0 &    1.0 & 34.0 \\
pds-100\_lp           &     156243 &     505360 &    1086785 &    26.7 &    9.5 &  2.8 \\
pds-40\_lp            &      66844 &     212859 &     462128 &     8.0 &    1.6 &  5.0 \\
% pds-40.mps\_lp        &      66844 &     212859 &     462128 &     8.0 &    2.0 &  4.0 \\
physiciansched3-3    &     266227 &      79555 &    1062479 &   256.2 &   12.0 & 21.4 \\
qap12\_lp             &       3192 &       8856 &      38304 &     3.0 &    0.3 & 10.0 \\
qap15\_lp             &       6330 &      22275 &      94950 &    32.0 &    1.0 & 32.0 \\
rail02               &      95791 &     270869 &     756228 &   316.0 &   42.0 &  7.5 \\
rail4284\_lp          &       4284 &    1092610 &   11279748 &    87.7 &   14.3 &  6.1 \\
rmine15\_lp           &     358395 &      42438 &     879732 &   413.1 &   28.0 & 14.8 \\
s100                 &      14733 &     364417 &    1777917 &    29.9 &    9.0 &  3.3 \\
s250r10              &      10962 &     273142 &    1318607 &    17.2 &    5.0 &  3.4 \\
s82\_lp               &      87878 &    1690631 &    7022608 &   637.3 &  107.5 &  5.9 \\
savsched1            &     295989 &     328575 &    1770507 &    75.4 &    5.0 & 15.1 \\
scpm1\_lp             &       5000 &     500000 &    6250000 &   185.5 &   17.1 & 10.8 \\
set-cover-model      &      10000 &    1102008 &   20442268 &  2327.9 &  105.0 & 22.2 \\
sgpf5y6\_lp           &     246077 &     308634 &     828070 &     0.5 &    0.3 &  1.7 \\
shs1023              &     133944 &     444625 &    1044725 &   160.2 &   17.0 &  9.4 \\
square41             &      40160 &      62234 &   13566426 &    24.4 &    2.0 & 12.2 \\
stat96v1\_lp          &       5995 &     197472 &     588798 &     9.0 &    5.3 &  1.7 \\
stat96v4\_lp          &       3173 &      62212 &     490472 &     1.9 &    0.3 &  6.3 \\
stormG2\_1000\_lp      &     528185 &    1259121 &    3341696 &    80.5 &   17.7 &  4.5 \\
stormg2-125\_lp       &      66185 &     157496 &     418321 &     3.0 &    0.8 &  3.8 \\
stp3d\_lp             &     159488 &     204880 &     662128 &    49.1 &    5.8 &  8.5 \\
supportcase10        &     165684 &      14770 &     555082 &    37.0 &    4.1 &  9.0 \\
tpl-tub-ws1617\_lp    &    1154615 &     747601 &     472056 &   175.8 &   52.0 &  3.4 \\
watson\_2\_lp          &     352013 &     671861 &    1841028 &     9.4 &    3.8 &  2.5 \\
world\_lp             &      34506 &      32734 &     164470 &     4.0 &    0.9 &  4.4 \\
\hline
\end{tabular}
\label{tab:LP-instances}
\caption{Problem size, run times of virtual Best \oldS and \newS, and the ratio \oldS/\newS of LP instances - Part II}
\end{table}



==> MIP_table_tex_sorted.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
Name & nrows & ncols & nonzeros &  \oldS [s] &  \newS [s] & ratio  \\
\hline
acc-tight5           &       3052 &       1339 &      16134 &    2558 &      4 & 639.5 \\
aflow30a             &        479 &        842 &       2091 &      44 &      2 & 22.0 \\
air04                &        823 &       8904 &      72965 &      12 &      2 &  6.0 \\
biella1              &       1203 &       7328 &      71489 &    4191 &     34 & 123.3 \\
bienst2              &        576 &        505 &       2184 &    1546 &     11 & 140.6 \\
binkar10\_1           &       1026 &       2298 &       4496 &      12 &      1 & 12.0 \\
cap6000              &       2176 &       6000 &      48243 &      10 &      1 & 10.0 \\
cbs-cta              &      10112 &      24793 &      64388 &       3 &      1 &  3.0 \\
core2536-691         &       2539 &      15293 &     177739 &     773 &      8 & 96.6 \\
cov1075              &        637 &        120 &      14280 &    5450 &      1 & 5450.0 \\
dano3\_5              &       3202 &      13873 &      79655 &     255 &     50 &  5.1 \\
danoint              &        664 &        521 &       3232 &    2037 &    112 & 18.2 \\
decomp2              &      10765 &      14387 &      64073 &      34 &      1 & 34.0 \\
dfn-gwin-UUM         &        158 &        938 &       2632 &     194 &      6 & 32.3 \\
disctom              &        399 &      10000 &      30000 &     338 &      1 & 338.0 \\
drayage-100-23       &       4630 &      11090 &      41550 &       8 &      1 &  8.0 \\
eil33-2              &         32 &       4516 &      44243 &      16 &      1 & 16.0 \\
eilB101              &        100 &       2818 &      24120 &      62 &      7 &  8.9 \\
enlight\_hard         &        100 &        200 &        560 &     471 &      1 & 471.0 \\
exp-1-500-5-5        &        550 &        990 &       1980 &    2165 &      1 & 2165.0 \\
gen-ip002            &         24 &         41 &        922 &     501 &     64 &  7.8 \\
hypothyroid-k1       &       5195 &       2602 &     433884 &     166 &     11 & 15.1 \\
iis-100-0-cov        &       3831 &        100 &      22986 &    2717 &     93 & 29.2 \\
iis-pima-cov         &       7201 &        768 &      71941 &    1182 &     72 & 16.4 \\
istanbul-no-cutoff   &      20346 &       5282 &      71477 &     154 &     13 & 11.8 \\
k1mushroom           &      16419 &       8211 &    1697946 &    1774 &     70 & 25.3 \\
lectsched-4-obj      &      14163 &       7901 &      82428 &     234 &      1 & 234.0 \\
map10                &     328818 &     164547 &     549920 &    3675 &     45 & 81.7 \\
map16715-04          &     328818 &     164547 &     549920 &    3942 &     51 & 77.3 \\
map18                &     328818 &     164547 &     549920 &    1071 &     15 & 71.4 \\
map20                &     328818 &     164547 &     549920 &    1214 &     18 & 67.4 \\
markshare\_4\_0        &          4 &         34 &        123 &      20 &      1 & 20.0 \\
\hline
\end{tabular}
\label{tab:MIP-instances-1}
\caption{Problem size, run times of virtual Best \oldS and \newS, and the ratio \oldS/\newS of MIP instances - PART I}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
Name & nrows & ncols & nonzeros &  \oldS [s] &  \newS [s] & ratio  \\
\hline
mas74                &         13 &        151 &       1706 &     238 &     32 &  7.4 \\
mas76                &         12 &        151 &       1640 &      15 &      4 &  3.8 \\
mcsched              &       2107 &       1747 &       8088 &      37 &      6 &  6.2 \\
mik-250-20-75-4      &        195 &        270 &       9270 &      68 &      1 & 68.0 \\
mine-166-5           &       8429 &        830 &      19412 &    1271 &      1 & 1271.0 \\
misc07               &        212 &        260 &       8619 &      15 &      1 & 15.0 \\
mod011               &       4480 &      10975 &      22271 &      40 &      8 &  5.0 \\
mspp16               &     561657 &      29280 &   27678735 &    1355 &    111 & 12.2 \\
mzzv42z              &      10460 &      11717 &     151261 &    4273 &      1 & 4273.0 \\
n4-3                 &       1236 &       3596 &      14036 &    5972 &      6 & 995.3 \\
n5-3                 &       1062 &       2550 &       9900 &     389 &      1 & 389.0 \\
neos-1109824         &      28979 &       1520 &      89528 &     161 &      1 & 161.0 \\
neos-1122047         &      57791 &       5100 &     163640 &       2 &      2 &  1.0 \\
neos-1171448         &      13206 &       4914 &     131859 &       6 &      1 &  6.0 \\
neos-1171737         &       4179 &       2340 &      58620 &    3033 &      3 & 1011.0 \\
neos13               &      20852 &       1827 &     253842 &     135 &     14 &  9.6 \\
neos-1337307         &       5687 &       2840 &      30799 &    6600 &      2 & 3300.0 \\
neos-1582420         &      10180 &      10100 &      24814 &      10 &      2 &  5.0 \\
neos-1601936         &       3131 &       4446 &      72500 &    1171 &     19 & 61.6 \\
neos18               &      11402 &       3312 &      24614 &     296 &      2 & 148.0 \\
neos-3083819-nubu    &       4725 &       8644 &      24048 &      21 &      1 & 21.0 \\
neos-3402294-bobin   &     591076 &       2904 &    2034888 &    4000 &      5 & 800.0 \\
neos-4722843-widden  &     113555 &      77723 &     311529 &     758 &     27 & 28.1 \\
neos-4738912-atrato  &       1947 &       6216 &      19521 &     178 &     11 & 16.2 \\
neos-476283          &      10015 &      11915 &    3945693 &      59 &     41 &  1.4 \\
neos-5188808-nattai  &      29452 &      14544 &     133686 &    5255 &    120 & 43.8 \\
neos5                &         63 &         63 &       2016 &    1110 &      5 & 222.0 \\
neos-662469          &       1085 &      18235 &     200055 &    8866 &     24 & 369.4 \\
neos-686190          &       3664 &       3660 &      18085 &      22 &      3 &  7.3 \\
neos-827175          &      14187 &      32504 &     110790 &       4 &      1 &  4.0 \\
neos8                &      46324 &      23228 &     313180 &      13 &      1 & 13.0 \\
neos-860300          &        850 &       1385 &     384329 &      19 &      2 &  9.5 \\
neos-916792          &       1909 &       1474 &     134442 &    1737 &     30 & 57.9 \\
neos-933966          &      12047 &      31762 &     180618 &     172 &      4 & 43.0 \\
neos-934278          &      11495 &      23123 &     125577 &     220 &     11 & 20.0 \\
\hline
\end{tabular}
\label{tab:MIP-instances-2}
\caption{Problem size, run times of virtual Best  \oldS and \newS, and the ratio \oldS/\newS of MIP instances - PART II}
\end{table}

\begin{table}[htbp]
\centering
\footnotesize
\begin{tabular}{lrrrrrr}
\toprule
Name & nrows & ncols & nonzeros &  \oldS [s] &  \newS [s] & ratio  \\
\hline
neos-950242          &      34224 &       5760 &     104160 &      37 &      3 & 12.3 \\
neos-957323          &       3757 &      57756 &     499656 &      13 &      8 &  1.6 \\
neos-960392          &       4744 &      59376 &     189503 &      32 &      2 & 16.0 \\
netdiversion         &     119589 &     129180 &     615282 &    2781 &     45 & 61.8 \\
noswot               &        182 &        128 &        735 &    1820 &      2 & 910.0 \\
ns1116954            &     131991 &      12648 &     410582 &    2315 &      4 & 578.8 \\
nu25-pr12            &       2313 &       5868 &      17712 &      20 &      1 & 20.0 \\
nw04                 &         36 &      87482 &     636666 &       2 &      2 &  1.0 \\
opm2-z7-s2           &      31798 &       2023 &      79762 &     453 &     13 & 34.9 \\
p200x1188c           &       1388 &       2376 &       4752 &       5 &      1 &  5.0 \\
pk1                  &         45 &         86 &        915 &      21 &      4 &  5.2 \\
qap10                &       1820 &       4150 &      18200 &      18 &      3 &  6.0 \\
qiu                  &       1192 &        840 &       3432 &      72 &      1 & 72.0 \\
ran16x16             &        288 &        512 &       1024 &     514 &      4 & 128.5 \\
reblock67            &       2523 &        670 &       7495 &    6246 &     12 & 520.5 \\
rmatr100-p10         &       7260 &       7359 &      21877 &      24 &      4 &  6.0 \\
rmatr100-p5          &       8685 &       8784 &      26152 &      27 &      6 &  4.5 \\
roi2alpha3n4         &       1251 &       6816 &     878812 &     182 &     23 &  7.9 \\
rout                 &        291 &        556 &       2431 &    1126 &      1 & 1126.0 \\
seymour1             &       4944 &       1372 &      33549 &     330 &     10 & 33.0 \\
sp150x300d           &        450 &        600 &       1200 &       5 &      1 &  5.0 \\
sp98ir               &       1531 &       1680 &      71704 &      95 &      5 & 19.0 \\
supportcase26        &        870 &        436 &       2492 &    6790 &     47 & 144.5 \\
supportcase40        &      38192 &      16440 &     104420 &    2367 &    116 & 20.4 \\
supportcase7         &       6532 &     138844 &    2845545 &      35 &      4 &  8.8 \\
swath3               &        884 &       6805 &      34965 &     738 &      4 & 184.5 \\
tanglegram1          &      68342 &      34759 &     205026 &      46 &      1 & 46.0 \\
tbfp-network         &       2436 &      72747 &     215837 &     279 &     75 &  3.7 \\
tr12-30              &        750 &       1080 &       2508 &     848 &     31 & 27.4 \\
trento1              &       1265 &       7687 &      93571 &   40858 &    106 & 385.4 \\
triptim1             &      15706 &      30055 &     515436 &      47 &     19 &  2.5 \\
unitcal\_7            &      48939 &      25755 &     127595 &     137 &     10 & 13.7 \\
\hline
\end{tabular}
\label{tab:MIP-instances-3}
\caption{Problem size, run times of virtual Best \oldS and \newS, and the ratio  \oldS/\newS of MIP instances - PART III}
\end{table}


==> barrier-tab.tex <==
\begin{table}[htbp]
\centering
\sffamily
\footnotesize
\begin{tabular}{lrrrrr}
\toprule
Name	& Pentium-III [s]	& i7-9700 [s]&	FP ops & ratio \\
\midrule
stat96v4            &   51.3 &    1.1 &      1568948 &   46.6\\
stat96v1            &   53.7 &    1.2 &      4652727 &   44.8\\
sgpf5y6             &   73.5 &    1.9 &      5015266 &   38.7\\
ns1687037           & 2364.7 &   64.8 &    514095229 &   36.5\\
self                &  131.3 &    4.0 &    296296481 &   32.8\\
buildingenergy      &  275.8 &    9.6 &     96421062 &   28.7\\
l30                 &   19.5 &    0.7 &     12393214 &   27.9\\
ds-big              &  300.2 &   10.8 &    325826721 &   27.8\\
watson\_2            &  244.3 &    9.2 &     89302850 &   26.6\\
ken-18              &   55.0 &    2.1 &    114327047 &   26.2\\
stormg2-125         &  102.2 &    4.1 &    132870547 &   24.9\\
stormG2\_1000        & 1484.5 &   62.0 &   1058928547 &   23.9\\
neos2               &  164.1 &    7.2 &    703175995 &   22.8\\
neos                &  785.0 &   35.1 &   1863823427 &   22.4\\
cont11              &  288.0 &   12.9 &    883805922 &   22.3\\
dbic1               &  143.6 &    6.5 &    221156856 &   22.1\\
neos1               &  277.2 &   12.9 &   1233411113 &   21.5\\
world               &   95.0 &    4.5 &    132147914 &   21.1\\
mod2                &   85.4 &    4.1 &    121316442 &   20.8\\
cont1               &  142.2 &    6.9 &    552874552 &   20.6\\
rail4284            & 1565.8 &   78.1 &  11548460885 &   20.0\\
cont4               &  166.8 &    8.7 &    576905552 &   19.2\\
stp3d               & 1240.3 &   66.2 &  12653896419 &   18.7\\
lp22                &   42.4 &    2.3 &    457213109 &   18.4\\
pds-40              & 1017.9 &   56.0 &   6110558500 &   18.2\\
dano3mip            &   82.7 &    4.6 &    753841103 &   18.0\\
fome13              &  580.1 &   33.1 &   4419484775 &   17.5\\
gen4                &   83.1 &    4.8 &    786779150 &   17.3\\
fome12              &  279.4 &   16.2 &   2031572179 &   17.2\\
qap12               &   89.5 &    5.4 &   2104003644 &   16.6\\
neos3               & 1053.8 &   64.5 &  40598849111 &   16.3\\
nug15               &  598.2 &   37.2 &  16497188763 &   16.1\\
qap15               &  750.8 &   46.8 &  15958930050 &   16.0\\
\midrule
SGM(1)              &{\bf 221.9}&{\bf 10.6}&        & {\bf 21.0}\\
\bottomrule
\end{tabular}
\label{tab:cpx7-barrier}
\caption{Run time of barrier algorithm for \cplex 7 on a 870~MHz Pentium-III and on an empty 3.6~GHz i7-9700.
Column \emph{FP ops} is the \emph{total FP ops to factor}. The table is sorted by increasing speed-up ratio. As can be seen, a higher number of FP ops generally leads to a lower speed-up factor.}
\end{table}

==> neto-tab.tex <==
\todo{Alignment problem in the header}

\begin{table}[htbp]
\centering
\sffamily
\footnotesize
\begin{tabular}{lrrrrr}
\toprule
&&Pentium III&\multicolumn{3}{|c}{i7-9700}\\
&&\multicolumn{2}{c|}{\cplex 7.0}&\multicolumn{2}{c}{\cplex 12.10}\\
Name	&Iterations&	empty [s]	& empty [s]&	empty [s]&	loaded [s]\\
\midrule
16\_n14	&1,082,628&	1369.38	&47.70&	49.61&	81.52\\
i\_n13	&2,038,669&	954.99	&45.30&	46.82&	76.93\\
lo10	&1,403,624&	1086.99	&65.50&	64.84&	103.32\\
long15	&870,757&	1061.19	&62.32&	65.72&	93.88\\
netlarge1&	15,443,416&	2648.15	&118.54	&115.98&	323.30\\
netlarge2&	1,031,653&	670.74	&40.60	&42.90&	65.17\\
netlarge3&	2,090,956&	1374.62	&80.02	&80.08&	134.66\\
netlarge6&	643,226	&329.43	&8.52	&7.90&	23.05\\
road\_flow\_05\_WI\_a&	1,823,212	&534.76	&24.78&	24.56&	72.31\\
road\_flow\_05\_WI\_b&	1,202,741	&286.16	&13.52&	13.62&	39.81\\
road\_flow\_05\_WI\_c&	1,516,739	&399.15	&19.36&	18.47&	57.09\\
road\_flow\_07\_TX\_a&	6,217,176	&4369.91&	194.92&	194.00&	630.08\\
road\_flow\_07\_TX\_b&	6,528,061	&4702.96&	207.94&	206.38&	673.12\\
road\_flow\_07\_TX\_c&	6,538,286	&4570.84&	206.14&	205.96&	655.00\\
square15	&918,610&	1192.27	&72.60	&71.56&	111.16\\
wide15	&870,757	&1059.15&	62.30&	66.92	&99.60\\
\midrule
SGM(1)		&&{\bf 1145.92}	&{\bf 55.56}	& {\bf 55.83 }&	{\bf 121.10}\\
\bottomrule
\end{tabular}
\label{tab:network-simplex}
\caption{Run time of network simplex algorithm for \cplex 7 and \cplex 12, on a 870~MHz Pentium-III and on a 3.6~GHz i7-9700, on an otherwise empty machine and on a fully loaded system.}
\end{table}
